Reduced-order Modeling on a Near-term Quantum Computer

Quantum computing is an advancing area of research in which computer hardware and algorithms are developed to take advantage of quantum mechanical phenomena. In recent studies, quantum algorithms have shown promise in solving linear systems of equations as well as systems of linear ordinary differential equations (ODEs) and partial differential equations (PDEs). Reduced-order modeling (ROM) algorithms for studying fluid dynamics have shown success in identifying linear operators that can describe flowfields, where dynamic mode decomposition (DMD) is a particularly useful method in which a linear operator is identified from data. In this work, DMD is reformulated as an optimization problem to propagate the state of the linearized dynamical system on a quantum computer. Quadratic unconstrained binary optimization (QUBO), a technique for optimizing quadratic polynomials in binary variables, allows for quantum annealing algorithms to be applied. A quantum circuit model (quantum approximation optimization algorithm, QAOA) is utilized to obtain predictions of the state trajectories. Results are shown for the quantum-ROM predictions for flow over a 2D cylinder at Re = 220 and flow over a NACA0009 airfoil at Re = 500 and $\alpha = 15^\circ{}$. The quantum-ROM predictions are found to depend on the number of bits utilized for a fixed point representation and the truncation level of the DMD model. Comparisons with DMD predictions from a classical computer algorithm are made, as well as an analysis of the computational complexity and prospects for future, more fault-tolerant quantum computers.

==> DirectCircuit.tex <==
\section{``Direct" Quantum Circuit Implementation of DMD matrix Multiplication}\label{direct_quantum_circuit}

The square matrix $A$ obtained for the 2D airfoil case with $6$ modes:

\begin{equation}
\left(\begin{array}{rrrrrr}
9.214\cdot 10^{-1} &-3.844\cdot 10^{-1} &-4.609\cdot 10^{-4} &3.526\cdot 10^{-4} &-2.778\cdot 10^{-4} &3.324\cdot 10^{-4}\\
3.842\cdot 10^{-1} &9.250\cdot 10^{-1} &2.645\cdot 10^{-5} &1.609\cdot 10^{-4} &2.598\cdot 10^{-4} &7.491\cdot 10^{-5}\\
1.617\cdot 10^{-2} &5.243\cdot 10^{-3} &7.044\cdot 10^{-1} &-7.173\cdot 10^{-1} &6.009\cdot 10^{-3} &-1.851\cdot 10^{-3}\\
6.393\cdot 10^{-3} &3.756\cdot 10^{-3} &7.021\cdot 10^{-1} &7.048\cdot 10^{-1} &1.291\cdot 10^{-3} &1.340\cdot 10^{-3}\\
6.459\cdot 10^{-3} &-7.841\cdot 10^{-4} &-1.351\cdot 10^{-2} &1.006\cdot 10^{-2} &3.780\cdot 10^{-1} &-9.241\cdot 10^{-1}\\
-7.658\cdot 10^{-3} &-5.135 \cdot 10^{-3} &-1.350\cdot 10^{-2} &1.984\cdot 10^{-3} &9.275\cdot 10^{-1} &3.777\cdot 10^{-1}
\end{array}\right)
%
\end{equation}
is first transformed into the following $8\times 8$ matrix to faciliate quantum-circuit implementation:

\begin{equation}
\overline{A}=
\left(\begin{array}{rrrrrrrr}
a_{00} &a_{01} &a_{02} &a_{03} &a_{04} &a_{05} &0 &0\\
a_{10} &a_{11} &a_{12} &a_{13} &a_{14} &a_{15} &0 &0\\
a_{20} &a_{21} &a_{22} &a_{23} &a_{24} &a_{25} &0 &0\\
a_{30} &a_{31} &a_{32} &a_{33} &a_{34} &a_{35} &0 &0\\
a_{40} &a_{41} &a_{42} &a_{43} &a_{44} &a_{45} &0 &0\\
a_{50} &a_{51} &a_{52} &a_{53} &a_{54} &a_{55} &0 &0\\
%
0 &0 &0 &0 &0 &0 &1 &0\\
0 &0 &0 &0 &0 &0 &0 &1
\end{array}\right)
%
\label{eq_DMD_8x8}
\end{equation}

The quantum circuit implementation of the matrix-vector multiplication of the matrix in equation (\ref{eq_DMD_8x8}) with a vector of length $8$ representing the amplitudes of the modes (final two entries are to be initialized at $0$) is complicated by the factor that the matrix is non-unitary. Also, considering the structure of this matrix, there is no apparent structure that can be used. For example, the matrix is not in the form of a sparse banded matrix or a circulant matrix.

For this general matrix structure, the first step involves the creation of an {\it augmented matrix} of size $16\times 16$ for the considered $8 \times 8$ matrix here. Specifically, for a given matrix $\overline{A}$, it is assumed that we can build the circuit equivalent of the following unitary matrix by using an ancilla quantum register:

\begin{equation}
\mathcal{U} = \left(\begin{array}{cc}
\overline{A} &\bullet\\
\bullet &\bullet
\end{array}\right)
\end{equation}
where each ``$\bullet$" represents a matrix which has no special meaning and their dimensions may be different on the diagonal and off-diagonal of the matrix. When applied to any arbitrary $\ket{\psi}$ on the system register, the above matrix generates the following output state

\begin{equation}
\mathcal{U}\ket{{\bf 0}}\ket{\Psi} = \ket{\Psi_1} + \ket{{\bf 0}}\overline{A}\ket{\Psi}
\end{equation}

Here, $\ket{{\bf 0}}$ represents the first vector in the standard basis and $\ket{\Psi}_1$ is the part of the output in which the first register is not in state $\ket{0}$. When the first register is in state $\ket{0}$, the second register holds $\overline{A}\ket{\Psi}$. Therefore, $\mathcal{U}$ can be used to emulate the action of $\overline{A}$ an any arbitrary state $\ket{\Psi}$. This idea was used by Daskin et al.\cite{Kais2012} to create a programmable circuit design for unitary matrices. Daskin and Kais\cite{DaskinKais2016} presented a general framework to simulate non-unitary processes on ancilla-based quantum circuits in which the success probability is maximized by using a technique called oblivious amplitude amplification. This technique (partially) circumvents a key drawback of adding ancilla qubits to a circuit, i.e. the reduced likelihood obtaining the required output through quantum measurement. 

\subsection{Outline of algorithm for augmented $8\times 8$ matrix}

For the $8\times 8$ matrix $\overline{A}$ defined in equation (\ref{eq_DMD_8x8}), it can be seen that a minimum of $n_A = log_2(8)=3$ qubits is needed to define indices of each of the columns and rows. The augmented, unitary matrix used here is a $16\times 16$ matrix, such that this minimum increases to $n_A = log_2(16)=4$ qubits. These $4$ qubits are termed $\ket{qu3|qu2|qu1|qu0}$ in the present example. In the circuit implementation, we need a further $4+1 = 5$ ancilla qubits, which are labeled as $\ket{anc4|anc3|\ldots |anc0}$. These ancilla qubits are created on the left-hand side of the $9$-qubit register, so that $\ket{anc4}$ represents the most-significant qubit in the indexing of the degrees of freedom. 

The qubits are now initialized with the $8$ initial values encoded in the $8$ amplitudes of the quantum state indexed as: $\ket{00000|0|qu3|qu2|qu1|qu0}$, for $qu3$, $qu2$, $qu1$ and $qu0$ $\in [0, 1]$. Similarly, the $8$ initial values of the augmented part of the solution vector are encoded in the amplitudes of the quantum state indexed as: $\ket{00000|1|qu3|qu2|qu1|qu0}$, for $qu3$, $qu2$, $qu1$ and $qu0$ $\in [0, 1]$.

The algorithm then proceeds as follows:

\begin{enumerate}
\item Application of the Hadamard operator on qubits $\ket{anc4}$, $\ket{anc3}$, $\ket{anc2}$ and $\ket{anc1}$;
%
\item Application $5$ qubit-swap operations: $\ket{anc0}$ with $\ket{qu0}$, $\ket{anc0}$ with $\ket{qu1}$,
$\ket{anc0}$ with $\ket{qu2}$ and $\ket{anc0}$ with $\ket{qu3}$;
%
\item Application of the $V_f$ matrix (as termed by Kais), implemented using controlled rotation operations in the circuit-based implementation;
%
\item Application of the Hadamard operator on qubits $\ket{anc0}$, $\ket{qu3}$, $\ket{qu2}$ and $\ket{qu1}$.
\end{enumerate}

\subsection{Quantum circuit implementation of $V_f$ matrix}
%
The quantum circuit implementation of $V_f$ follows a row-by-row approach:
\begin{itemize}
    \item $16$ rows in the augmented matrix - in the quantum circuit implementation $4$ qubits act as 'control' to define which row is considered;
    \item For each row, $16$ elements are represented by $16$ controlled-rotation gates (where angle is defined by specific values of matrix elements) - the quantum circuit implementation employs $4$ qubits as control qubits to index the considered matrix element (i.e. define which of $16$ elements on the considered row is implemented by rotation gate);
    \item Therefore, for the considered example: $16\times 16$ controlled rotation gates - each controlled by $4+4=8$ qubits.
\end{itemize}

Starting from this ``baseline" implementation with $8$ controls acting on rotation gates, additional ancillae qubits will be needed to implement the controlled rotations with a reduced control qubits (i.e. reduction to a single or two control qubits).
